A global convergence theory for deep ReLU implicit networks via over-parameterization

Implicit deep learning has received increasing attention recently due to the fact that it generalizes the recursive prediction rules of many commonly used neural network architectures. Its prediction rule is provided implicitly based on the solution of an equilibrium equation. Although a line of recent empirical studies has demonstrated its superior performances, the theoretical understanding of implicit neural networks is limited. In general, the equilibrium equation may not be well-posed during the training. As a result, there is no guarantee that a vanilla (stochastic) gradient descent (SGD) training nonlinear implicit neural networks can converge. This paper fills the gap by analyzing the gradient flow of Rectified Linear Unit (ReLU) activated implicit neural networks. For an $m$-width implicit neural network with ReLU activation and $n$ training samples, we show that a randomly initialized gradient descent converges to a global minimum at a linear rate for the square loss function if the implicit neural network is \textit{over-parameterized}. It is worth noting that, unlike existing works on the convergence of (S)GD on finite-layer over-parameterized neural networks, our convergence results hold for implicit neural networks, where the number of layers is \textit{infinite}.

==> Sec2_Preliminaries/Sec2_Preliminaries.tex <==
% !TEX root = ../implicit_nn.tex

\section{Notations}
%We begin with an introduction to the notations. 
Given a vector $\vx$, $\norm{\vx}$ is the Euclidean norm of $\vx$. Given a matrix $\mA$, $\norm{\mA}$ is the operator norm of $\mA$. 
If $\mA$ is square matrix, then $\lambda_{\min}(\mA)$ and $\lambda_{\max}(\mA)$ denote the smallest and largest eigenvalue of $\mA$, respectively, and $\lambda_{\max}(\mA) = \norm{\mA}$. We denote $[n]\triangleq\{1,2,\cdots, n\}$.

%Let $\{(\vx_i, y_i)\}_{i=1}^{n}$ be a training dataset with $n$ samples, where $\vx_i\in \reals^d$ is the input vector, and $y_i\in \reals$ is the label. In this paper, we consider an implicit neural networks with the transition at the $\ell$-th layer in the following form:
%\begin{align}
%	\vz^{\ell} = \sigma(\tilde{\gamma}\mA \vz^{\ell-1} +\phi(\vx)),
%	\label{eq:transition}
%\end{align}
%where $\vz^{\ell}\in \reals^m$ is the output of the $\ell$-th layer, $\mA\in \reals^{m\times m}$ is the trainable parameter matrix, the positive number $\tilde{\gamma}\triangleq\gamma/\sqrt{m}$ for some $\gamma\in (0,1)$ is utilized to scale the matrix $\mA$ to ensure the existence of the equilibrium point $\vz^{*}=\lim_{\ell\rightarrow \infty}\vz^{\ell}$, which we discuss later in Section~\ref{sec:forward}), $\sigma(u)=\max\{0, u\}$ is the ReLU activation function, and the function $\phi: \reals^{d}\rightarrow \reals^{m}$ is the feature map that transform the input vector $\vx$ to the desired feature vector $\vphi\triangleq \phi(\vx)$. Here we consider a simple nonlinear feature map $\phi$ given by
%\begin{align}
%	\phi(\vx) \triangleq  \frac{1}{\sqrt{m}}\sigma(\mW\vx), \label{eq:phi def}
%\end{align}
%where $\mW\in \reals^{m\times d}$ is another trainable parameter matrix. 
%\textcolor{blue}{The implicit neural networks are considered as an \textit{infinitely} deep network by letting $\ell\rightarrow \infty$.
%The vector $\vz^*$ is not only the limit of the sequence $\{\vz^{\ell}\}_{\ell=0}^{\infty}$ with $\vz_0 = \0$, but it is also the \textit{equilibrium point} or \textit{fixed point} of the equilibrium equation as follows
%\begin{align}
%	\vz^* = \sigma(\tilde{\gamma}\mA \vz^* + \vphi ).
%	\label{eq:equilibrium equation}
%\end{align}
%In implicit neural networks, the prediction $\hat{y}$ for the input vector $\vx$ is the combination of the fixed point $\vz^*$ and the feature vector $\vphi$, \ie,
%\begin{align}
%	\hat{y}=\vu^T\vz^*  +\vv^T \vphi,\label{eq:prediction}
%\end{align}
%where $\vu, \vv\in \reals^m$ are trainable weight vectors.
%We denote $\vtheta \triangleq \vect{\mA, \mW, \vu, \vv}$ as all the training parameters.
%Along with the square loss as the loss function, \ie, $\ell(\hat{y}, y) = \frac{1}{2}\ell(\hat{y} - y)^2$, the objective function or the total loss $L(\vtheta)$ is given by
%\begin{align}
%	L(\vtheta) = \sum_{i=1}^n \ell(\hat{y}_i, y_i)
%	=\frac{1}{2}\norm{\hat{\vy} - \vy}^2,
%\end{align}
%where $\hat{\vy}$ and $\vy$ are the vectors of stacking all the prediction and labels.}



